RSK bases and Kazhdan-Lusztig cells

From the combinatorial characterizations of the right, left, and two-sided Kazhdan-Lusztig cells of the symmetric group, 'RSK bases' are constructed for certain quotients by two-sided ideals of the group ring and the Hecke algebra. Applications to invariant theory, over various base rings, of the general linear group and representation theory of the symmetric group are discussed.

==> old-intro.tex <==


In Theorems~\ref{t:klbasis}
and~\ref{t:p2kl} of~\S\ref{s:proof} 
we deduce from this observation more good properties of
the Kazhdan-Lusztig $C$-basis with respect to representations.
%The proof of these
%characterizations,  however,  is  matter.


The reasoning in the previous paragraph
might seem like putting the cart before the horse,
for the proofs in~\cite{geck} of the combinatorial characterizations
proceed by first establishing---by means of the Murphy basis---the
observation above (if only implicitly).   
Our defense rests on the following:
\begin{itemize}
\item The arguments in~\S\ref{s:proof} are formal and simple.
In particular,  they don't need any such extra construct as
the Murphy basis.
\item The combinatorial characterizations admit other approaches,
notwithstanding the fact that proofs for some of them are at 
present available only in~\cite{geck}.
\end{itemize}

%The Hecke algebra analogues of some definitions and preliminary 
In~\S\ref{s:notation}  we recall---from~\cite{kl,dj,mp,geck}---definitions, 
notation, and preliminary results to be used in~\S\S\ref{s:notation}--\ref{s:poschar}.

In \S\ref{s:hanalogues}  we generalize the results of~\S\ref{s:motivation}:
Theorem~\ref{t:htabloidl} %in~\S\ref{s:hanalogues} 
is a Hecke algebra analogue
%or characteristic free version 
of Theorem~\ref{t:tabloidl};  and Theorem~\ref{t:cfreemlin} is %similarly 
a characteristic free version
of the result over~$\fieldc$ on multilinear invariants stated 
in~\S\ref{s:motivation} and proved in~\S\ref{s:proof}.  

In~\S\ref{s:matrixg} we work out, more explicitly than in~\S\ref{s:proof},
what the combinatorial characterizations mean for the action of 
$C$-basis elements indexed by permutations of a certain~\shape~$\lambda$
on the right cell module associated to~$\lambda$.   The action
is conveniently encoded by the matrix~$\matrixgl$ of~(\ref{e:cprod}).
The determinant of~$\matrixgl$ is shown in~\S\ref{s:gandgram}, 
using results of~\cite{dj,mp},
to be related to the determinant~$\gramdet$ %---called the 
%{\em Gram determinant\/}---
of the matrix of the 
Dipper-James bilinear form on the Specht module~$\spechtl$ with respect
to the `standard basis'.   In~\cite[Theorem~4.11]{dj}, there is a formula
for~$\gramdet$ in terms of hook lengths.
Combining it with a result from~\cite{jmathas},
a similar hook length formula
is obtained for~$\det\matrixgl$ in \S\ref{s:gdet} (Theorem~\ref{t:formula}).   
Our formula is nicer than the one in~\cite[Theorem~4.11]{dj}
in that there is no obtruding power of the indeterminate:
see the proof of Theorem~\ref{t:formula} for how that power vanishes.\footnote{
The obtruding sign factor in our formula too 
goes away if we work with the $C'$-basis
instead of the $C$-basis.
}


Apart from any interest the results of~\S\S\ref{s:matrixg}--\ref{s:gdet}
may have in themselves, they have the following 
applications as described in~\S\ref{s:poschar}:
\begin{itemize}
\item 
They provide another approach to one half of the 
Carter conjecture about irreducibility of Specht modules under 
specializations---see Theorem~\ref{t:cpirred}.
\item 
We obtain generalizations (to not necessarily semi-simple situations)
of Theorems~\ref{p:klbasis},~\ref{p:p2kl}---see
Theorems~\ref{t:cpklbasis},~\ref{t:cpp2kl}.
\end{itemize}
\subsection*{Acknowledgments}  Thanks to the {\sffamily GAP\/} 
program, computations performed on which were useful in 
formulating the results;  to the 
{\sffamily Abdus Salam International Centre
for Theoretical Physics\/},  during a visit to which of one
of the authors much of this work was brought to completion;
to the {\sffamily Skype\/} program, using which the authors
were able to stay in touch during that visit.


==> part4.tex <==
\textbf{ The matrix $\matrixgl$ and its determinant}

Let $\lambda$ be a fixed partition of $n$. We associate to this
$\lambda$, a matrix $\matrixgl$, which gives ``a multiplication
table modulo lower cells'' for the~$C_w$ of $\shape~\lambda$. This
matrix also contains information on the action of the $C$-basis
elements indexed by permutations of $\shape~\lambda$, on the right
cell module $\rcmodl$.  We are thus motivated to studying the
properties of this matrix.  Towards achieving this, we relate the
matrix $\matrixgl$ to the matrix of the ``Dipper-James bilinear form''
on $\rcmodl$. By doing so, we are able to obtain a relation between
the Gram determinant (recalled in \S\ref{s:gandgram} and the
determinant of $\matrixgl$. In \S\ref{s:gdet}, we obtain a formula for
this determinant which comes essentially from a known formula for the
Gram determinant. This we do more for the sake of completion and in
the faith that the choice of the $C$-basis on $\rcmodl$ is more
appropriate. This we feel is justified by the ``hook
formula''(see formula\ref{t:formula}) which takes a neat form, without any
obtrusive powers.

As an application of these results, we illustrate in \S\ref{s:poschar}
another way of proving one half of the Carter Conjecture. This comes
from the fact that the determinant of $\matrixgl$ being non-zero
implies linear independence of the $C_w$'s of $\shape~\lambda$. We
also give Hecke analogues of Theorems \ref{t:klbasis}, \ref{t:p2kl}.

